ViR:the Vision Reservoir

The most recent year has witnessed the success of applying the Vision Transformer (ViT) for image classification. However, there are still evidences indicating that ViT often suffers following two aspects, i) the high computation and the memory burden from applying the multiple Transformer layers for pre-training on a large-scale dataset, ii) the over-fitting when training on small datasets from scratch. To address these problems, a novel method, namely, Vision Reservoir computing (ViR), is proposed here for image classification, as a parallel to ViT. By splitting each image into a sequence of tokens with fixed length, the ViR constructs a pure reservoir with a nearly fully connected topology to replace the Transformer module in ViT. Two kinds of deep ViR models are subsequently proposed to enhance the network performance. Comparative experiments between the ViR and the ViT are carried out on several image classification benchmarks. Without any pre-training process, the ViR outperforms the ViT in terms of both model and computational complexity. Specifically, the number of parameters of the ViR is about 15% even 5% of the ViT, and the memory footprint is about 20% to 40% of the ViT. The superiority of the ViR performance is explained by Small-World characteristics, Lyapunov exponents, and memory capacity.

==> backup_bib <==
@String(PAMI = {IEEE Trans. Pattern Anal. Mach. Intell.})
@String(IJCV = {Int. J. Comput. Vis.})
@String(CVPR= {IEEE Conf. Comput. Vis. Pattern Recog.})
@String(ICCV= {Int. Conf. Comput. Vis.})
@String(ECCV= {Eur. Conf. Comput. Vis.})
@String(NIPS= {Adv. Neural Inform. Process. Syst.})
@String(ICPR = {Int. Conf. Pattern Recog.})
@String(BMVC= {Brit. Mach. Vis. Conf.})
@String(TOG= {ACM Trans. Graph.})
@String(TIP  = {IEEE Trans. Image Process.})
@String(TVCG  = {IEEE Trans. Vis. Comput. Graph.})
@String(TMM  = {IEEE Trans. Multimedia})
@String(ACMMM= {ACM Int. Conf. Multimedia})
@String(ICME = {Int. Conf. Multimedia and Expo})
@String(ICASSP=	{ICASSP})
@String(ICIP = {IEEE Int. Conf. Image Process.})
@String(ACCV  = {ACCV})
@String(ICLR = {Int. Conf. Learn. Represent.})
@String(IJCAI = {IJCAI})
@String(PR   = {Pattern Recognition})
@String(AAAI = {AAAI})
@String(CVPRW= {IEEE Conf. Comput. Vis. Pattern Recog. Worksh.})
@String(CSVT = {IEEE Trans. Circuit Syst. Video Technol.})

@String(SPL	= {IEEE Sign. Process. Letters})
@String(VR   = {Vis. Res.})
@String(JOV	 = {J. Vis.})
@String(TVC  = {The Vis. Comput.})
@String(JCST  = {J. Comput. Sci. Tech.})
@String(CGF  = {Comput. Graph. Forum})
@String(CVM = {Computational Visual Media})


@String(PAMI  = {IEEE TPAMI})
@String(IJCV  = {IJCV})
@String(CVPR  = {CVPR})
@String(ICCV  = {ICCV})
@String(ECCV  = {ECCV})
@String(NIPS  = {NeurIPS})
@String(ICPR  = {ICPR})
@String(BMVC  =	{BMVC})
@String(TOG   = {ACM TOG})
@String(TIP   = {IEEE TIP})
@String(TVCG  = {IEEE TVCG})
@String(TCSVT = {IEEE TCSVT})
@String(TMM   =	{IEEE TMM})
@String(ACMMM = {ACM MM})
@String(ICME  =	{ICME})
@String(ICASSP=	{ICASSP})
@String(ICIP  = {ICIP})
@String(ACCV  = {ACCV})
@String(ICLR  = {ICLR})
@String(IJCAI = {IJCAI})
@String(PR = {PR})
@String(AAAI = {AAAI})
@String(CVPRW= {CVPRW})
@String(CSVT = {IEEE TCSVT})



@misc{Authors14,
 author = {FirstName LastName},
 title = {The frobnicatable foo filter},
 note = {Face and Gesture submission ID 324. Supplied as supplemental material {\tt fg324.pdf}},
 year = 2014
}

@misc{Authors14b,
 author = {FirstName LastName},
 title = {Frobnication tutorial},
 note = {Supplied as supplemental material {\tt tr.pdf}},
 year = 2014
}

@article{Alpher02,
author = {FirstName Alpher},
title = {Frobnication},
journal = PAMI,
volume = 12,
number = 1,
pages = {234--778},
year = 2002
}

@article{Alpher03,
author = {FirstName Alpher and  FirstName Fotheringham-Smythe},
title = {Frobnication revisited},
journal = {Journal of Foo},
volume = 13,
number = 1,
pages = {234--778},
year = 2003
}
@inproceedings{choromanski2020rethinking_iclr,
  title={Rethinking Attention with Performers},
  author={Choromanski, Krzysztof Marcin and Likhosherstov, Valerii and Dohan, David and Song, Xingyou and Gane, Andreea and Sarlos, Tamas and Hawkins, Peter and Davis, Jared Quincy and Mohiuddin, Afroz and Kaiser, Lukasz and others},
  booktitle={International Conference on Learning Representations},
  year={2020}
}
@article{Alpher04,
author = {FirstName Alpher and FirstName Fotheringham-Smythe and FirstName Gamow},
title = {Can a machine frobnicate?},
journal = {Journal of Foo},
volume = 14,
number = 1,
pages = {234--778},
year = 2004
}

@inproceedings{Alpher05,
author = {FirstName Alpher and FirstName Gamow},
title = {Can a computer frobnicate?},
booktitle = CVPR,
pages = {234--778},
year = 2005
}


@article{lukovsevivcius2009reservoir,
  title={Reservoir computing approaches to recurrent neural network training},
  author={Luko{\v{s}}evi{\v{c}}ius, Mantas and Jaeger, Herbert},
  journal={Computer Science Review},
  volume={3},
  number={3},
  pages={127--149},
  year={2009},
  publisher={Elsevier}
}

@article{gallicchio2020deep,
  title={Deep randomized neural networks},
  author={Gallicchio, Claudio and Scardapane, Simone},
  journal={Recent Trends in Learning From Data},
  pages={43--68},
  year={2020},
  publisher={Springer, Cham}
}

@article{li2021localvit,
  title={Localvit: Bringing locality to vision transformers},
  author={Li, Yawei and Zhang, Kai and Cao, Jiezhang and Timofte, Radu and Van Gool, Luc},
  journal={arXiv preprint arXiv:2104.05707},
  year={2021}
}

@article{jaeger2001echo,
  title={The “echo state” approach to analysing and training recurrent neural networks-with an erratum note},
  author={Jaeger, Herbert},
  journal={Bonn, Germany: German National Research Center for Information Technology GMD Technical Report},
  volume={148},
  number={34},
  pages={13},
  year={2001},
  publisher={Bonn}
}


@article{jaeger2004harnessing,
  title={Harnessing nonlinearity: Predicting chaotic systems and saving energy in wireless communication},
  author={Jaeger, Herbert and Haas, Harald},
  journal={science},
  volume={304},
  number={5667},
  pages={78--80},
  year={2004},
  publisher={American Association for the Advancement of Science}
}


@article{maass2002real,
  title={Real-time computing without stable states: A new framework for neural computation based on perturbations},
  author={Maass, Wolfgang and Natschl{\"a}ger, Thomas and Markram, Henry},
  journal={Neural computation},
  volume={14},
  number={11},
  pages={2531--2560},
  year={2002},
  publisher={MIT Press}
}


@article{tino2001predicting,
  title={Predicting the future of discrete sequences from fractal representations of the past},
  author={Tino, Peter and Dorffner, Georg},
  journal={Machine Learning},
  volume={45},
  number={2},
  pages={187--217},
  year={2001},
  publisher={Springer}
}


@article{jaeger2007optimization,
  title={Optimization and applications of echo state networks with leaky-integrator neurons},
  author={Jaeger, Herbert and Luko{\v{s}}evi{\v{c}}ius, Mantas and Popovici, Dan and Siewert, Udo},
  journal={Neural networks},
  volume={20},
  number={3},
  pages={335--352},
  year={2007},
  publisher={Elsevier}
}


@article{maass2014noise,
  title={Noise as a resource for computation and learning in networks of spiking neurons},
  author={Maass, Wolfgang},
  journal={Proceedings of the IEEE},
  volume={102},
  number={5},
  pages={860--880},
  year={2014},
  publisher={IEEE}
}


@article{verzelli2021learn,
  title={Learn to synchronize, synchronize to learn},
  author={Verzelli, Pietro and Alippi, Cesare and Livi, Lorenzo},
  journal={Chaos: An Interdisciplinary Journal of Nonlinear Science},
  volume={31},
  number={8},
  pages={083119},
  year={2021},
  publisher={AIP Publishing LLC}
}


@article{rodan2010minimum,
  title={Minimum complexity echo state network},
  author={Rodan, Ali and Tino, Peter},
  journal={IEEE transactions on neural networks},
  volume={22},
  number={1},
  pages={131--144},
  year={2010},
  publisher={IEEE}
}


@article{rodan2012simple,
  title={Simple deterministically constructed cycle reservoirs with regular jumps},
  author={Rodan, Ali and Ti{\v{n}}o, Peter},
  journal={Neural computation},
  volume={24},
  number={7},
  pages={1822--1852},
  year={2012},
  publisher={MIT Press}
}


@article{verzelli2021input,
  title={Input-to-State Representation in Linear Reservoirs Dynamics},
  author={Verzelli, Pietro and Alippi, Cesare and Livi, Lorenzo and Ti{\v{n}}o, Peter},
  journal={IEEE Transactions on Neural Networks and Learning Systems},
  year={2021},
  publisher={IEEE}
}


@article{farkavs2016computational,
  title={Computational analysis of memory capacity in echo state networks},
  author={Farka{\v{s}}, Igor and Bos{\'a}k, Radom{\'\i}r and Gergel', Peter},
  journal={Neural Networks},
  volume={83},
  pages={109--120},
  year={2016},
  publisher={Elsevier}
}


@article{livi2017determination,
  title={Determination of the edge of criticality in echo state networks through Fisher information maximization},
  author={Livi, Lorenzo and Bianchi, Filippo Maria and Alippi, Cesare},
  journal={IEEE transactions on neural networks and learning systems},
  volume={29},
  number={3},
  pages={706--717},
  year={2017},
  publisher={IEEE}
}


@article{sussillo2009generating,
  title={Generating coherent patterns of activity from chaotic neural networks},
  author={Sussillo, David and Abbott, Larry F},
  journal={Neuron},
  volume={63},
  number={4},
  pages={544--557},
  year={2009},
  publisher={Elsevier}
}


@article{hoerzer2014emergence,
  title={Emergence of complex computational structures from chaotic neural networks through reward-modulated Hebbian learning},
  author={Hoerzer, Gregor M and Legenstein, Robert and Maass, Wolfgang},
  journal={Cerebral cortex},
  volume={24},
  number={3},
  pages={677--690},
  year={2014},
  publisher={Oxford University Press}
}


@article{pyle2019reservoir,
  title={A reservoir computing model of reward-modulated motor learning and automaticity},
  author={Pyle, Ryan and Rosenbaum, Robert},
  journal={Neural computation},
  volume={31},
  number={7},
  pages={1430--1461},
  year={2019},
  publisher={MIT Press One Rogers Street, Cambridge, MA 02142-1209, USA journals-info~…}
}

@article{gallicchio2017deep1,
  title={Deep echo state network (deepesn): A brief survey},
  author={Gallicchio, Claudio and Micheli, Alessio},
  journal={arXiv preprint arXiv:1712.04323},
  year={2017}
}

@inproceedings{liu2018analysis,
  title={Analysis of memory capacity for deep echo state networks},
  author={Liu, Xuanlin and Chen, Mingzhe and Yin, Changchuan and Saad, Walid},
  booktitle={2018 17th IEEE International Conference on Machine Learning and Applications (ICMLA)},
  pages={443--448},
  year={2018},
  organization={IEEE}
}


@article{gallicchio2017deep2,
  title={Deep reservoir computing: A critical experimental analysis},
  author={Gallicchio, Claudio and Micheli, Alessio and Pedrelli, Luca},
  journal={Neurocomputing},
  volume={268},
  pages={87--99},
  year={2017},
  publisher={Elsevier}
}


@inproceedings{zhou2020deep,
  title={Deep reservoir computing meets 5g mimo-ofdm systems in symbol detection},
  author={Zhou, Zhou and Liu, Lingjia and Chandrasekhar, Vikram and Zhang, Jianzhong and Yi, Yang},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={34},
  number={01},
  pages={1266--1273},
  year={2020}
}


@article{dutoit2009pruning,
  title={Pruning and regularization in reservoir computing},
  author={Dutoit, Xavier and Schrauwen, Benjamin and Van Campenhout, Jan and Stroobandt, Dirk and Van Brussel, Hendrik and Nuttin, Marnix},
  journal={Neurocomputing},
  volume={72},
  number={7-9},
  pages={1534--1546},
  year={2009},
  publisher={Elsevier}
}


@article{xue2007decoupled,
  title={Decoupled echo state networks with lateral inhibition},
  author={Xue, Yanbo and Yang, Le and Haykin, Simon},
  journal={Neural Networks},
  volume={20},
  number={3},
  pages={365--376},
  year={2007},
  publisher={Elsevier}
}


@article{deng2007collective,
  title={Collective behavior of a small-world recurrent neural system with scale-free distribution},
  author={Deng, Zhidong and Zhang, Yi},
  journal={IEEE Transactions on neural networks},
  volume={18},
  number={5},
  pages={1364--1375},
  year={2007},
  publisher={IEEE}
}


@techreport{jaeger2007discovering,
  title={Discovering multiscale dynamical features with hierarchical echo state networks},
  author={Jaeger, Herbert},
  year={2007},
  institution={Jacobs University Bremen}
}


@inproceedings{skowronski2006minimum,
  title={Minimum mean squared error time series classification using an echo state network prediction model},
  author={Skowronski, Mark D and Harris, John G},
  booktitle={2006 IEEE International Symposium on Circuits and Systems},
  pages={4--pp},
  year={2006},
  organization={IEEE}
}


@article{aswolinskiy2018time,
  title={Time series classification in reservoir-and model-space},
  author={Aswolinskiy, Witali and Reinhart, Ren{\'e} Felix and Steil, Jochen},
  journal={Neural Processing Letters},
  volume={48},
  number={2},
  pages={789--809},
  year={2018},
  publisher={Springer}
}


@inproceedings{schaetti2016echo,
  title={Echo state networks-based reservoir computing for mnist handwritten digits recognition},
  author={Schaetti, Nils and Salomon, Michel and Couturier, Rapha{\"e}l},
  booktitle={2016 IEEE Intl Conference on Computational Science and Engineering (CSE) and IEEE Intl Conference on Embedded and Ubiquitous Computing (EUC) and 15th Intl Symposium on Distributed Computing and Applications for Business Engineering (DCABES)},
  pages={484--491},
  year={2016},
  organization={IEEE}
}

@book{nakajima2021reservoir_book,
  title={Reservoir Computing},
  author={Nakajima, Kohei and Fischer, Ingo},
  year={2021},
  publisher={Springer}
}

@inproceedings{tong2018reservoir,
  title={Reservoir computing with untrained convolutional neural networks for image recognition},
  author={Tong, Zhiqiang and Tanaka, Gouhei},
  booktitle={2018 24th International Conference on Pattern Recognition (ICPR)},
  pages={1289--1294},
  year={2018},
  organization={IEEE}
}


@article{chang2020reinforcement,
  title={Reinforcement learning with convolutional reservoir computing},
  author={Chang, Hanten and Futagami, Katsuya},
  journal={Applied Intelligence},
  volume={50},
  number={8},
  pages={2400--2410},
  year={2020},
  publisher={Springer}
}


@article{mosleh2017brain,
  title={Brain-inspired wireless communications: Where reservoir computing meets MIMO-OFDM},
  author={Mosleh, Somayeh Susanna and Liu, Lingjia and Sahin, Cenk and Zheng, Yahong Rosa and Yi, Yang},
  journal={IEEE transactions on neural networks and learning systems},
  volume={29},
  number={10},
  pages={4694--4708},
  year={2017},
  publisher={IEEE}
}


@article{hamedani2017reservoir,
  title={Reservoir computing meets smart grids: Attack detection using delayed feedback networks},
  author={Hamedani, Kian and Liu, Lingjia and Atat, Rachad and Wu, Jinsong and Yi, Yang},
  journal={IEEE Transactions on Industrial Informatics},
  volume={14},
  number={2},
  pages={734--743},
  year={2017},
  publisher={IEEE}
}

@article{van2017advances_Nanophotonics,
  title={Advances in photonic reservoir computing},
  author={Van der Sande, Guy and Brunner, Daniel and Soriano, Miguel C},
  journal={Nanophotonics},
  volume={6},
  number={3},
  pages={561--576},
  year={2017},
  publisher={De Gruyter}
}

@article{brunner2019photonic,
  title={Photonic reservoir computing},
  author={Brunner, Daniel and Soriano, Miguel C and Van der Sande, Guy},
  journal={De Gruyter},
  volume={8},
  pages={19},
  year={2019}
}

@article{tanaka2019recent,
  title={Recent advances in physical reservoir computing: A review},
  author={Tanaka, Gouhei and Yamane, Toshiyuki and H{\'e}roux, Jean Benoit and Nakane, Ryosho and Kanazawa, Naoki and Takeda, Seiji and Numata, Hidetoshi and Nakano, Daiju and Hirose, Akira},
  journal={Neural Networks},
  volume={115},
  pages={100--123},
  year={2019},
  publisher={Elsevier}
}

@inproceedings{wang2021end_cvpr,
  title={End-to-end video instance segmentation with transformers},
  author={Wang, Yuqing and Xu, Zhaoliang and Wang, Xinlong and Shen, Chunhua and Cheng, Baoshan and Shen, Hao and Xia, Huaxia},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={8741--8750},
  year={2021}
}

@inproceedings{chen2021transformer_cvpr,
  title={Transformer tracking},
  author={Chen, Xin and Yan, Bin and Zhu, Jiawen and Wang, Dong and Yang, Xiaoyun and Lu, Huchuan},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={8126--8135},
  year={2021}
}

@article{dosovitskiy2020image,
  title={An image is worth 16x16 words: Transformers for image recognition at scale},
  author={Dosovitskiy, Alexey and Beyer, Lucas and Kolesnikov, Alexander and Weissenborn, Dirk and Zhai, Xiaohua and Unterthiner, Thomas and Dehghani, Mostafa and Minderer, Matthias and Heigold, Georg and Gelly, Sylvain and others},
  journal={arXiv preprint arXiv:2010.11929},
  year={2020}
}


@article{willoughby1979solutions,
  title={Solutions of ill-posed problems (AN Tikhonov and VY Arsenin)},
  author={Willoughby, Ralph A},
  journal={SIAM Review},
  volume={21},
  number={2},
  pages={266},
  year={1979},
  publisher={Society for Industrial and Applied Mathematics}
}


@inproceedings{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  booktitle={Advances in neural information processing systems},
  pages={5998--6008},
  year={2017}
}

@article{hopfield1982neural,
  title={Neural networks and physical systems with emergent collective computational abilities},
  author={Hopfield, John J},
  journal={Proceedings of the national academy of sciences},
  volume={79},
  number={8},
  pages={2554--2558},
  year={1982},
  publisher={National Acad Sciences}
}

@book{jaeger2002tutorial,
  title={Tutorial on training recurrent neural networks, covering BPPT, RTRL, EKF and the" echo state network" approach},
  author={Jaeger, Herbert},
  volume={5},
  number={01},
  year={2002},
  publisher={GMD-Forschungszentrum Informationstechnik Bonn}
}

@article{lun2015novel,
  title={A novel model of leaky integrator echo state network for time-series prediction},
  author={Lun, Shu-Xian and Yao, Xian-Shuang and Qi, Hong-Yun and Hu, Hai-Feng},
  journal={Neurocomputing},
  volume={159},
  pages={58--66},
  year={2015},
  publisher={Elsevier}
}

@article{maass1997networks,
  title={Networks of spiking neurons: the third generation of neural network models},
  author={Maass, Wolfgang},
  journal={Neural networks},
  volume={10},
  number={9},
  pages={1659--1671},
  year={1997},
  publisher={Elsevier}
}

@article{ardalani2010chaotic,
  title={Chaotic time series prediction with residual analysis method using hybrid Elman--NARX neural networks},
  author={Ardalani-Farsa, Muhammad and Zolfaghari, Saeed},
  journal={Neurocomputing},
  volume={73},
  number={13-15},
  pages={2540--2553},
  year={2010},
  publisher={Elsevier}
}

@article{legenstein2007edge,
  title={Edge of chaos and prediction of computational performance for neural circuit models},
  author={Legenstein, Robert and Maass, Wolfgang},
  journal={Neural networks},
  volume={20},
  number={3},
  pages={323--334},
  year={2007},
  publisher={Elsevier}
}

@article{basterrech2017echo,
  title={Echo state queueing networks: a combination of reservoir computing and random neural networks},
  author={Basterrech, Sebasti{\'a}n and Rubino, Gerardo},
  journal={Probability in the Engineering and Informational Sciences},
  volume={31},
  number={4},
  pages={457--476},
  year={2017},
  publisher={Cambridge University Press}
}

@article{wang2015optimizing,
  title={Optimizing the echo state network with a binary particle swarm optimization algorithm},
  author={Wang, Heshan and Yan, Xuefeng},
  journal={Knowledge-Based Systems},
  volume={86},
  pages={182--193},
  year={2015},
  publisher={Elsevier}
}

@article{carroll2021low,
  title={Low dimensional manifolds in reservoir computers},
  author={Carroll, TL},
  journal={Chaos: An Interdisciplinary Journal of Nonlinear Science},
  volume={31},
  number={4},
  pages={043113},
  year={2021},
  publisher={AIP Publishing LLC}
}

@article{koster2021master,
  title={Master memory function for delay-based reservoir computers with single-variable dynamics},
  author={K{\"o}ster, Felix and Yanchuk, Serhiy and L{\"u}dge, Kathy},
  journal={arXiv preprint arXiv:2108.12643},
  year={2021}
}

@inproceedings{kleyko2017modality,
  title={Modality classification of medical images with distributed representations based on cellular automata reservoir computing},
  author={Kleyko, Denis and Khan, Sumeer and Osipov, Evgeny and Yong, Suet-Peng},
  booktitle={2017 IEEE 14th International Symposium on Biomedical Imaging (ISBI 2017)},
  pages={1053--1056},
  year={2017},
  organization={IEEE}
}

@article{jalalvand2018application,
  title={On the application of reservoir computing networks for noisy image recognition},
  author={Jalalvand, Azarakhsh and Demuynck, Kris and De Neve, Wesley and Martens, Jean-Pierre},
  journal={Neurocomputing},
  volume={277},
  pages={237--248},
  year={2018},
  publisher={Elsevier}
}

@article{koprinkova2021reservoir,
  title={Reservoir Computing Approach for Gray Images Segmentation},
  author={Koprinkova-Hristova, Petia},
  journal={arXiv preprint arXiv:2107.11077},
  year={2021}
}


@article{Shen2020ReservoirT,
  title={Reservoir Transformer},
  author={Sheng Shen and Alexei Baevski and Ari S. Morcos and Kurt Keutzer and Michael Auli and Douwe Kiela},
  journal={ArXiv},
  year={2020},
  volume={abs/2012.15045}
}

@article{lukovsevivcius2012reservoir,
  title={Reservoir computing trends},
  author={Luko{\v{s}}evi{\v{c}}ius, Mantas and Jaeger, Herbert and Schrauwen, Benjamin},
  journal={KI-K{\"u}nstliche Intelligenz},
  volume={26},
  number={4},
  pages={365--371},
  year={2012},
  publisher={Springer}
}

@article{shi2007support,
  title={Support vector echo-state machine for chaotic time-series prediction},
  author={Shi, Zhiwei and Han, Min},
  journal={IEEE transactions on neural networks},
  volume={18},
  number={2},
  pages={359--372},
  year={2007},
  publisher={IEEE}
}

@article{min2010multivariate,
  title={Multivariate time series online predictor with Kalman filter trained reservoir},
  author={Min, Han and Ya-Nan, Wang},
  journal={Acta Automatica Sinica},
  volume={36},
  number={1},
  pages={169--173},
  year={2010}
}

@inproceedings{ozturk2005computing,
  title={Computing with transiently stable states},
  author={Ozturk, Mustafa C and Principe, Jose C},
  booktitle={Proceedings. 2005 IEEE International Joint Conference on Neural Networks, 2005.},
  volume={3},
  pages={1467--1472},
  year={2005},
  organization={IEEE}
}

@inproceedings{touvron2021training,
  title={Training data-efficient image transformers \& distillation through attention},
  author={Touvron, Hugo and Cord, Matthieu and Douze, Matthijs and Massa, Francisco and Sablayrolles, Alexandre and J{\'e}gou, Herv{\'e}},
  booktitle={International Conference on Machine Learning},
  pages={10347--10357},
  year={2021},
  organization={PMLR}
}

@article{chaudhari2021attentive,
  title={An attentive survey of attention models},
  author={Chaudhari, Sneha and Mithal, Varun and Polatkan, Gungor and Ramanath, Rohan},
  journal={ACM Transactions on Intelligent Systems and Technology (TIST)},
  volume={12},
  number={5},
  pages={1--32},
  year={2021},
  publisher={ACM New York, NY}
}

@article{correia2021attention,
  title={Attention, please! A survey of Neural Attention Models in Deep Learning},
  author={Correia, Alana de Santana and Colombini, Esther Luna},
  journal={arXiv preprint arXiv:2103.16775},
  year={2021}
}

@article{khan2021transformers,
  title={Transformers in vision: A survey},
  author={Khan, Salman and Naseer, Muzammal and Hayat, Munawar and Zamir, Syed Waqas and Khan, Fahad Shahbaz and Shah, Mubarak},
  journal={arXiv preprint arXiv:2101.01169},
  year={2021}
}

@article{wang2021pyramid,
  title={Pyramid vision transformer: A versatile backbone for dense prediction without convolutions},
  author={Wang, Wenhai and Xie, Enze and Li, Xiang and Fan, Deng-Ping and Song, Kaitao and Liang, Ding and Lu, Tong and Luo, Ping and Shao, Ling},
  journal={arXiv preprint arXiv:2102.12122},
  year={2021}
}


@article{Yuan2021TokenstoTokenVT,
  title={Tokens-to-Token ViT: Training Vision Transformers from Scratch on ImageNet},
  author={Li Yuan and Yunpeng Chen and Tao Wang and Weihao Yu and Yujun Shi and Francis E. H. Tay and Jiashi Feng and Shuicheng Yan},
  journal={ArXiv},
  year={2021},
  volume={abs/2101.11986}
}

@article{2012Learning,
  title={Learning Multiple Layers of Features from Tiny Images},
  author={ Krizhevsky, Alex },
  year={2012},
}

@article{hendrycks2019benchmarking,
  title={Benchmarking neural network robustness to common corruptions and perturbations},
  author={Hendrycks, Dan and Dietterich, Thomas},
  journal={arXiv preprint arXiv:1903.12261},
  year={2019}
}

@article{newman2003structure,
  title={The structure and function of complex networks},
  author={Newman, Mark EJ},
  journal={SIAM review},
  volume={45},
  number={2},
  pages={167--256},
  year={2003},
  publisher={SIAM}
}

@article{watts1998collective,
  title={Collective dynamics of ‘small-world’networks},
  author={Watts, Duncan J and Strogatz, Steven H},
  journal={nature},
  volume={393},
  number={6684},
  pages={440--442},
  year={1998},
  publisher={Nature Publishing Group}
}

@article{albert2002statistical,
  title={Statistical mechanics of complex networks},
  author={Albert, R{\'e}ka and Barab{\'a}si, Albert-L{\'a}szl{\'o}},
  journal={Reviews of modern physics},
  volume={74},
  number={1},
  pages={47},
  year={2002},
  publisher={APS}
}

@article{humphries2006brainstem,
  title={The brainstem reticular formation is a small-world, not scale-free, network},
  author={Humphries, Mark D and Gurney, Kevin and Prescott, Tony J},
  journal={Proceedings of the Royal Society B: Biological Sciences},
  volume={273},
  number={1585},
  pages={503--511},
  year={2006},
  publisher={The Royal Society London}
}


@article{kawai2019small,
  title={A small-world topology enhances the echo state property and signal propagation in reservoir computing},
  author={Kawai, Yuji and Park, Jihoon and Asada, Minoru},
  journal={Neural Networks},
  volume={112},
  pages={15--23},
  year={2019},
  publisher={Elsevier}
}

@article{rubinov2015wiring,
  title={Wiring cost and topological participation of the mouse brain connectome},
  author={Rubinov, Mikail and Ypma, Rolf JF and Watson, Charles and Bullmore, Edward T},
  journal={Proceedings of the National Academy of Sciences},
  volume={112},
  number={32},
  pages={10032--10037},
  year={2015},
  publisher={National Acad Sciences}
}

@article{bertschinger2004real,
  title={Real-time computation at the edge of chaos in recurrent neural networks},
  author={Bertschinger, Nils and Natschl{\"a}ger, Thomas},
  journal={Neural computation},
  volume={16},
  number={7},
  pages={1413--1436},
  year={2004},
  publisher={MIT Press}
}

@article{boedecker2012information,
  title={Information processing in echo state networks at the edge of chaos},
  author={Boedecker, Joschka and Obst, Oliver and Lizier, Joseph T and Mayer, N Michael and Asada, Minoru},
  journal={Theory in Biosciences},
  volume={131},
  number={3},
  pages={205--213},
  year={2012},
  publisher={Springer}
}

@inproceedings{verstraeten2010memory,
  title={Memory versus non-linearity in reservoirs},
  author={Verstraeten, David and Dambre, Joni and Dutoit, Xavier and Schrauwen, Benjamin},
  booktitle={The 2010 international joint conference on neural networks (IJCNN)},
  pages={1--8},
  year={2010},
  organization={IEEE}
}

@article{shimada1979numerical,
  title={A numerical approach to ergodic problem of dissipative dynamical systems},
  author={Shimada, Ippei and Nagashima, Tomomasa},
  journal={Progress of theoretical physics},
  volume={61},
  number={6},
  pages={1605--1616},
  year={1979},
  publisher={Oxford University Press}
}

@book{jaeger2001short,
  title={Short term memory in echo state networks},
  author={Jaeger, Herbert and others},
  volume={5},
  year={2001},
  publisher={GMD-Forschungszentrum Informationstechnik}
}

@article{hendrycks2016gaussian,
  title={Gaussian error linear units (gelus)},
  author={Hendrycks, Dan and Gimpel, Kevin},
  journal={arXiv preprint arXiv:1606.08415},
  year={2016}
}
